Learning from Noisy Labels with Deep Neural Networks: A Survey

Deep learning has achieved remarkable success in numerous domains with help from large amounts of big data. However, the quality of data labels is a concern because of the lack of high-quality labels in many real-world scenarios. As noisy labels severely degrade the generalization performance of deep neural networks, learning from noisy labels (robust training) is becoming an important task in modern deep learning applications. In this survey, we first describe the problem of learning with label noise from a supervised learning perspective. Next, we provide a comprehensive review of 62 state-of-the-art robust training methods, all of which are categorized into five groups according to their methodological difference, followed by a systematic comparison of six properties used to evaluate their superiority. Subsequently, we perform an in-depth analysis of noise rate estimation and summarize the typically used evaluation methodology, including public noisy datasets and evaluation metrics. Finally, we present several promising research directions that can serve as a guideline for future studies. All the contents will be available at https://github.com/songhwanjun/Awesome-Noisy-Labels.

==> backup.tex <==
\hfill mds
 
\hfill August 26, 2015

\subsection{Subsection Heading Here}
Subsection text here.

% needed in second column of first page if using \IEEEpubid
%\IEEEpubidadjcol

\subsubsection{Subsubsection Heading Here}
Subsubsection text here.


% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.




\section{Conclusion}
The conclusion goes here.





% if have a single appendix:
%\appendix[Proof of the Zonklar Equations]
% or
%\appendix  % for no appendix heading
% do not use \section anymore after \appendix, only \section*
% is possibly needed

% use appendices with more than one appendix
% then use \section to start each appendix
% you must declare a \section before using any
% \subsection or using \label (\appendices by itself
% starts a section numbered zero.)
%


\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...

\newcolumntype{L}[1]{>{\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{X}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}

\begin{table*}[t!]
\centering
\caption{Comparison of robust deep learning approaches for noisy labels.}
\begin{tabular}{|L{2.2cm} L{2.85cm}||X{1.4cm}|X{1.55cm}|X{1.8cm}|X{1.65cm}|X{1.5cm}|X{1.6cm}|}
\hline
%\multicolumn{2}{|>{}c|}{} & {P1} & {P2} & {P3} & {P4} & {P5} & {P6} & {P7} \\\hline
\multicolumn{2}{|>{}c||}{\textbf{Categorization}} & \!\!\!\textbf{Flexibility}\!\!\! & \!\!\!\textbf{No Pre-train}\!\!\! & \!\!\!\textbf{Full Exploration}\!\!\! & \!\!\!\textbf{No Supervision}\!\!\!  & \!\!\!\textbf{Heavy Noise}\!\!\! & \!\!\!\textbf{Complex Noise}\!\!\! \\\hline\hline
\multicolumn{2}{|>{}c||}{\hspace*{-3.2cm}Robust Loss Function }& O & O & O & O  & X & X\\\hline
\multirow{2}{*}
{\hspace*{-0.1cm}Robust Architecture\!\!}
& \!\!Noise Adaptation Layer & $\Delta$ & O & O & O  & X & X\\
\cline{2-8}
& \!\!Self-designed Architecture\!\!\! & X & $\Delta$ & O & X  & $\Delta$ & O\\ \hline
\multicolumn{2}{|>{}c||}{\hspace*{-3.15cm}Robust Regularization }& O & $\Delta$ & O & O & $\Delta$ & $\Delta$ \\\hline
\multirow{2}{*}
{\hspace*{-0.08cm}\vspace*{-0.35cm}Loss Adjustment}
& \!\!Loss Correction & O & $\Delta$ & O & X  & X & X\\
\cline{2-8}
& \!\!Loss Reweighting & O & O & O & O  & X & $\Delta$\\
\cline{2-8}
& \!\!Label Refurbishment & O & O & O & $\Delta$ & X & $\Delta$\\ \hline
\multicolumn{2}{|>{}c||}{\hspace*{-3.65cm}Sample Selection}& O & O & X & $\Delta$ & O & $\Delta$ \\\hline
\multirow{2}{*}
{\hspace*{-0.07cm}Meta Learning}
& \!\!Fast Adaption & O & O & O & X & $\Delta$ & O\\
\cline{2-8}
& \!\!Learning to Update & O & O & O & X & $\Delta$ & O\\ \hline
\multicolumn{2}{|>{}c||}{\hspace*{-2.6cm}Semi-supervised Learning}& O & $\Delta$ & O & O & O & $\Delta$ \\\hline
\end{tabular}
\label{fig:typeDistribution}
\end{table*}


{
\newcolumntype{L}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{X}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{Y}[1]{>{\let\newline\\\arraybackslash\hspace{1pt}}m{#1}}


\begin{table*}[h]
\vspace*{-0.2cm}
\caption{Comparison of all proposed methods for overcoming noisy labels.}
\vspace*{-0.2cm}
\begin{tabular}{L{0.7cm}|L{2.5cm}|Y{4.7cm}|X{0.5cm}|X{0.5cm}|X{0.5cm}|X{0.5cm}|X{0.5cm}|X{0.5cm}|Y{2.9cm}}
\toprule
\multicolumn{2}{c|}{\textbf{Direction}} & \hspace*{2.0cm}\textbf{Method} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P6} & \!\!\!\textbf{Implementation}\!\! \\ \hline
\multicolumn{2}{c|}{\multirow{4}{*}{{\makecell[l]{Robust Loss Function\\\hspace*{0.75cm}(\textsection \ref{sec:robust_loss_function})}}}}  
& \emph{Robust MAP}\cite{ghosh2017robust} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & N/A \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Generalized Cross Entropy}\cite{zhang2018generalized} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & Unofficial\,(PyTorch)\protect\footnotemark[1] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Symmetric Cross Entropy}\cite{wang2019symmetric} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & Official\,(Keras)\protect\footnotemark[2] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Curriculum Learning}\cite{lyu2020curriculum} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{red!10}\cmark & \cellcolor{red!10}$\bigtriangleup$ & N/A \\\midrule

\multirow{9}{*}{\hspace*{0.13cm}\!\!\!\!\!\!\rotatebox[origin=c]{90}{\makecell[l]{Robust Architecture\\\hspace*{0.66cm}(\textsection \ref{sec:robust_architecture})}}\!\!\!\!\!} & \multirow{6}{*}{\makecell[l]{Noisy Adaptation\\\hspace*{0.67cm}Layer}}  
& \emph{Webly Learning}\cite{chen2015webly} & \cellcolor{gray!10}$\bigtriangleup$ & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & Official\,(Caffe)\protect\footnotemark[3] \\\cline{3-10}
& & \emph{Noise Model}\cite{sukhbaatar2014training} & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & Unofficial\,(Keras)\protect\footnotemark[4] \\\cline{3-10}
& & \emph{Dropout Noise Model}\cite{jindal2016learning} & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & Official\,(MATLAB)\protect\footnotemark[5] \\\cline{3-10}
& & \emph{s-model}\cite{goldberger2017training} & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & Official\,(Keras)\protect\footnotemark[6]\\\cline{3-10}
& & \emph{c-model}\cite{goldberger2017training} & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\cmark & Official\,(Keras)\protect\footnotemark[6] \\\cline{3-10}
& & \emph{NLNN}\cite{bekker2016training} & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & Unofficial\,(Chainer)\protect\footnotemark[7] \\\cmidrule{2-10}

& \multirow{3}{*}{\makecell[l]{Self-designed\\\hspace*{0.06cm}Architecture}} 
& \emph{Probablistic Noise Model}\cite{xiao2015learning} & \cellcolor{red!10}\xmark & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & $ \cellcolor{gray!10}\bigtriangleup$ & \cellcolor{blue!10}\cmark & Official\,(Caffe)\protect\footnotemark[8] \\\cline{3-10}
& & \emph{Masking}\cite{han2018masking} & \cellcolor{red!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & $ \cellcolor{gray!10}\bigtriangleup$ & \cellcolor{blue!10}\cmark & Official\,(TensorFlow)\protect\footnotemark[9] \\\cline{3-10}
& & \emph{Contrastive-Additive Noise Network}\cite{yao2018deep} & \cellcolor{red!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark &\cellcolor{red!10} \cmark & $ \cellcolor{gray!10}\bigtriangleup$ &\cellcolor{blue!10} \cmark & N/A \\\midrule

\multicolumn{2}{c|}{\multirow{6}{*}{{\makecell[l]{Robust Regularization\\\hspace*{0.75cm}(\textsection \ref{sec:robust_regularization})}}}} 
& \emph{Adversarial Training}\cite{goodfellow2014explaining} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{gray!10}$ \bigtriangleup$ & Unofficial\,(PyTorch)\protect\footnotemark[10] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Label Smoothing}\cite{pereyra2017regularizing} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{gray!10}$ \bigtriangleup$ & Unofficial\,(PyTorch)\protect\footnotemark[11] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Mixup}\cite{zhang2018mixup} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(PyTorch)\protect\footnotemark[12] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Bilevel Learning}\cite{jenni2018deep} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(TensorFlow)\protect\footnotemark[13] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Annotator Confusion}\cite{tanno2019learning} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(TensorFlow)\protect\footnotemark[14] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Pre-training}\cite{hendrycks2019using} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(PyTorch)\protect\footnotemark[15] \\\midrule

\multirow{9}{*}{\hspace*{0.13cm}\!\!\!\!\!\!\rotatebox[origin=c]{90}{\makecell[l]{Loss Adjustment\\\hspace*{0.5cm}(\textsection \ref{sec:loss_adjustment})}}\!\!\!\!\!} & \multirow{3}{*}{\makecell[l]{Loss Correction}}  
& \emph{Backward Correction}\cite{patrini2017making} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark &  \cellcolor{red!10}\xmark &  \cellcolor{red!10}\xmark &  \cellcolor{red!10}\xmark & Official\,(Keras)\protect\footnotemark[16] \\\cline{3-10}
& & \emph{Forward Correction}\cite{patrini2017making} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark &  \cellcolor{red!10}\xmark &  \cellcolor{red!10}\xmark &  \cellcolor{red!10}\xmark & Official\,(Keras)\protect\footnotemark[16] \\\cline{3-10}
& & \emph{Gold Loss Correction}\cite{hendrycks2018using} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\cmark &  \cellcolor{red!10}\xmark &  \cellcolor{red!10}\xmark &  \cellcolor{red!10}\xmark & Official\,(PyTorch)\protect\footnotemark[17] \\\cmidrule{2-10}

& \multirow{2}{*}{\makecell[l]{Loss Reweigting}} 
& \emph{Importance Reweighting}\cite{wang2017multiclass} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & Unofficial\,(PyTorch)\protect\footnotemark[18] \\\cline{3-10}
& & \emph{Active Bias}\cite{chang2017active} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & Unofficial\,(TensorFlow)\protect\footnotemark[19]\!\! \\\cmidrule{2-10}

& \multirow{4}{*}{\makecell[l]{Label Refurbishment}} & \emph{Bootstrapping}\cite{reed2015training} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\xmark & \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & Unofficial\,(Keras)\protect\footnotemark[20] \\\cline{3-10}
& & \emph{Dynamic Bootstrapping}\cite{arazo2019unsupervised} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(PyTorch)\protect\footnotemark[21] \\\cline{3-10}
& & \emph{D2L}\cite{ma2018dimensionality} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(Keras)\protect\footnotemark[22] \\\cline{3-10}
& & \emph{SELFIE}\cite{song2019selfie} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\xmark & \cellcolor{red!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(TensorFlow)\protect\footnotemark[23] \\\midrule

\multicolumn{2}{c|}{\multirow{7}{*}{{\makecell[l]{Sample Selection\\\hspace*{0.53cm}(\textsection \ref{sec:sample_selection})}}}}  & \emph{Decouple}\cite{malach2017decoupling} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(TensorFlow)\protect\footnotemark[24] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{MentorNet}\cite{jiang2018mentornet} & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\xmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(TensorFlow)\protect\footnotemark[25] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Co-teaching}\cite{han2018co} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(PyTorch)\protect\footnotemark[26] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Co-teaching+}\cite{yu2019does} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(PyTorch)\protect\footnotemark[27] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Iterative Detection}\cite{wang2018iterative} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(Keras)\protect\footnotemark[28] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{ITLM}\cite{shen2019learning} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(GluonCV)\protect\footnotemark[29] \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{INCV}\cite{chen2019understanding} & \cellcolor{blue!10}\cmark &\cellcolor{blue!10} \cmark & \cellcolor{red!10}\xmark & \cellcolor{red!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(Keras)\protect\footnotemark[30] \\\midrule

\multirow{7}{*}{\hspace*{0.13cm}\!\!\!\!\!\!\rotatebox[origin=c]{90}{\makecell[l]{Meta Learning\\\hspace*{0.38cm}(\textsection \ref{sec:meta_learning})}}\!\!\!\!\!} & \multirow{2}{*}{\makecell[l]{Fast Adaption}}  
& \emph{Meta-Regressor}\cite{garcia2016noise} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\xmark & \cellcolor{gray!10}\cmark & \cellcolor{blue!10}\cmark & Official\,(R)\protect\footnotemark[31] \\\cline{3-10}
& & \emph{MLNT}\cite{li2019learning} & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{gray!10}\xmark & \cellcolor{blue!10}\cmark & Official\,(PyTorch)\protect\footnotemark[32] \\\cmidrule{2-10}%\cline{2-10}

& \multirow{5}{*}{\makecell[l]{Learning to Update}} 
& \emph{Knowledge Distillation}\cite{li2017learning} & \cellcolor{gray!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\cmark &  \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & N/A \\\cline{3-10}
& & \emph{L2LWS}\cite{dehghani2017learning} & \cellcolor{gray!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark &  \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & Unofficial\,(TensorFlow)\protect\footnotemark[33]\!\! \\\cline{3-10}
& & \emph{CWS}\cite{dehghani2017avoiding} & \cellcolor{gray!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark &  \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & N/A \\\cline{3-10}
& & \emph{Automatic Reweighting}\cite{ren2018learning} & \cellcolor{gray!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark &  \cellcolor{red!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & Official\,(TensorFlow)\protect\footnotemark[34] \\\cline{3-10}
& & \emph{Meta-Weight-Net}\cite{shu2019meta} & \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{red!10}\xmark &  \cellcolor{gray!10}$ \bigtriangleup$ & \cellcolor{blue!10}\cmark & Official\,(PyTorch)\protect\footnotemark[35] \\\midrule

\multicolumn{2}{c|}{\multirow{4}{*}{{\makecell[l]{Semi-supervised\\\hspace*{-0.02cm}Learning (\textsection \ref{sec:sample_selection})}}}}  
& \emph{Label Aggregation}\cite{yan2016robust} & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\xmark & \cellcolor{blue!10}\xmark & \cellcolor{gray!10}$ \bigtriangleup$ & N/A \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{Two-Stage Framework}\cite{ding2018semi} & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\xmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & N/A \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{SELF}\cite{nguyen2020self} & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & N/A \\\cline{3-10}
\multicolumn{2}{c|}{} & \emph{DivideMix}\cite{li2020dividemix} & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{blue!10}\cmark & \cellcolor{gray!10}$ \bigtriangleup$ & Official\,(PyTorch)\protect\footnotemark[36] \\\bottomrule
\end{tabular}
\vspace*{-0.9cm}
\end{table*}

}
